CheMatAgent: Enhancing LLMs for Chemistry and Materials Science through Tree-Search Based Tool Learning

Large language models (LLMs) have recently demonstrated promising capabilities in chemistry tasks while still facing challenges due to outdated pretraining knowledge and the difficulty of incorporating specialized chemical expertise. To address these issues, we propose an LLM-based agent that synergistically integrates 137 external chemical tools created ranging from basic information retrieval to complex reaction predictions, and a dataset curation pipeline to generate the dataset ChemToolBench that facilitates both effective tool selection and precise parameter filling during fine-tuning and evaluation. We introduce a Hierarchical Evolutionary Monte Carlo Tree Search (HE-MCTS) framework, enabling independent optimization of tool planning and execution. By leveraging self-generated data, our approach supports step-level fine-tuning (FT) of the policy model and training task-adaptive PRM and ORM that surpass GPT-4o. Experimental evaluations demonstrate that our approach significantly improves performance in Chemistry QA and discovery tasks, offering a robust solution to integrate specialized tools with LLMs for advanced chemical applications. All datasets and code are available at https://github.com/AI4Chem/ChemistryAgent .

==> figures/mcts_result.tex <==
\begin{figure*}[htb]
  \centering
  \includegraphics[width=1.0\linewidth]{assets/mcts_result.png}
  \caption{Mcts result}
  \label{fig:mcts_result}
\end{figure*}

==> sections/acknowledgements.tex <==
\section*{Acknowledgments}

/

==> tables/dataset_analysis.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htb]
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lrccc}
\toprule
\textbf{Dataset} & \textbf{Amount} & \textbf{Finetuning} & \textbf{Benchmark} & \textbf{Type} \\
\midrule
\textbf{ChemCrow} & 22 & {\color{red}\ding{56}} & {\color[HTML]{008114}\ding{52}} & Multiple \\
\textbf{CACTUS} & 1000 & {\color{red}\ding{56}} & {\color[HTML]{008114}\ding{52}} & Single \\
\textbf{Ours} & & & & \\
\qquad\textbf{-Chemistry} & 12,444 & {\color[HTML]{008114}\ding{52}} & {\color[HTML]{008114}\ding{52}} & Single + Multiple \\
\qquad\textbf{-Materials} & 17,365 & {\color[HTML]{008114}\ding{52}} & {\color[HTML]{008114}\ding{52}} & Single + Multiple \\
\bottomrule
\end{tabular}
}
\caption{Dataset Comparison}
\label{table:dataset}
\end{table}

==> tables/exp_multi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[htb]
% \caption{multiple}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lccccccccccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multirow{2}{*}{\textbf{Format}} & \multicolumn{3}{c}{\textbf{Tool}}  & \multicolumn{3}{c}{\textbf{Param}}  & \multicolumn{3}{c}{\textbf{Return}}  & \multirow{2}{*}{\textbf{Pass Rate}} \\
% \multicolumn{1}{c}{}  &  & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} &  \\
% \midrule
% \textbf{GPT-4o-mini} & 99.83 & 83.22 & 78.86 & 80.98 & 76.04 & 72.19 & 74.06 & 77.05 & 73.13 & 75.04 & 58.00 \\
% \textbf{Claude-3.5-S} & 97.42 & 83.64 & 85.37 & 84.50 & 76.03 & 77.53 & 76.77 & 74.96 & 78.54 & 76.71 & 57.00 \\
% \textbf{ChemLLM*} & 98.10 & 76.84 & 88.08 & 82.07 & 68.22 & 80.20 & 73.72 & 68.84 & 80.45 & 74.19 & 53.00 \\
% \textbf{Qwen-2.5-7B-I} & 51.25 & 64.15 & 41.81 & 50.63 & 56.48 & 37.36 & 44.97 & 29.25 & 37.20 & 32.75 & 22.50 \\
% \textbf{Llama-2-7B-C} & 9.50 & 33.33 & 3.50 & 6.33 & 20.48 & 2.39 & 4.28 & 2.45 & 2.70 & 2.57 & 8.50 \\
% \textbf{Llama-3.1-8B-I} & 75.99 & 59.95 & 38.31 & 46.75 & 52.98 & 33.71 & 41.20 & 40.83 & 34.34 & 37.31 & 15.00 \\
% \textbf{Llama-3.1-8B-I*} & 99.20 & 93.10 & 92.21 & 92.65 & 83.85 & 83.15 & 83.50 & 85.03 & 84.90 & 84.96 & 55.00 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[htb]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multirow{2}{*}{\textbf{Format}} & \multicolumn{3}{c}{\textbf{Tool}}  & \multicolumn{3}{c}{\textbf{Param}}  & \multicolumn{3}{c}{\textbf{Return}}  & \multirow{2}{*}{\textbf{Pass Rate}} \\
\multicolumn{1}{c}{}  &  & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} &  \\
\midrule
\textbf{GPT-4o-mini} & 99.83 & 83.22 & 78.86 & 80.98 & 76.04 & 72.19 & 74.06 & 77.05 & 73.13 & 75.04 & 58.00 \\
\textbf{Claude-3.5-S} & 97.42 & 83.64 & 85.37 & 84.50 & 76.03 & 77.53 & 76.77 & 74.96 & 78.54 & 76.71 & 57.00 \\
\textbf{ChemLLM*} & 98.10 & 76.84 & 88.08 & 82.07 & 68.22 & 80.20 & 73.72 & 68.84 & 80.45 & 74.19 & 53.00 \\
\textbf{Qwen-2.5-7B-I} & 51.25 & 64.15 & 41.81 & 50.63 & 56.48 & 37.36 & 44.97 & 29.25 & 37.20 & 32.75 & 22.50 \\
\textbf{Llama-2-7B-C} & 9.50 & 33.33 & 3.50 & 6.33 & 20.48 & 2.39 & 4.28 & 2.45 & 2.70 & 2.57 & 8.50 \\
\textbf{Llama-3.1-8B-I} & 75.99 & 59.95 & 38.31 & 46.75 & 52.98 & 33.71 & 41.20 & 40.83 & 34.34 & 37.31 & 15.00 \\
\textbf{Llama-3.1-8B-I*} & 99.20 & 93.10 & 92.21 & 92.65 & 83.85 & 83.15 & 83.50 & 85.03 & 84.90 & 84.96 & 55.00 \\
\midrule


\textbf{GPT-4o-mini-M} & / & 85.06 & 83.57 & 84.31 & 88.47 & / & / & 75.97 & 74.64 & 75.30 & 62.30 \\
\textbf{Claude-3.5-S-M} & / & 89.80 & 86.27 & 88.00 & 86.36 & / & / & 77.55 & 74.51 & 76.00 & 57.06 \\

\textbf{Qwen-2.5-7B-M1} & / & 89.30 & 82.63 & 85.83 & 86.89 & / & / & 77.89 & 72.08 & 74.87 & 62.00 \\
\textbf{Qwen-2.5-7B-M2} & / & 90.01 & 83.33 & 86.54 & 88.40 & / & / & 79.89 & 74.07 & 76.92 & 58.33 \\
\textbf{Qwen-2.5-7B-M3} & / & 91.14 & 90.45 & 90.80 & 89.32 & / & / & 81.41 & 80.79 & 81.10 & 67.32 \\

\textbf{Llama-3.1-8B-M0} & / & 75.45 & 78.45 & 76.92 & 85.25 & / & / & 65.09 & 67.68 & 66.36 & 29.19 \\
\textbf{Llama-3.1-8B-M1} & / & 87.74 & 87.32 & 87.53 & 85.92 & / & / & 75.81 & 75.44 & 75.62 & 69.50 \\
\textbf{Llama-3.1-8B-M2} & / & 93.18 & 88.39 & 90.79 & 95.12 & / & / & 88.64 & 84.07 & 86.36 & 72.30 \\
\textbf{Llama-3.1-8B-M3} & / & 93.22 & 91.73 & 92.47 & 92.36 & / & / & 86.09 & 84.72 & 85.41 & 72.20 \\

\bottomrule
\end{tabular}
}
\caption{Main Results on the Multiple-Tool-Calling Comprehensive Chemistry Benchmark.}
\label{table:exp_main}
\end{table*}





